HPA-MPC: Hybrid Perception-Aware Nonlinear Model Predictive Control for Quadrotors with Suspended Loads

Quadrotors equipped with cable-suspended loads represent a versatile, low-cost, and energy efficient solution for aerial transportation, construction, and manipulation tasks. However, their real-world deployment is hindered by several challenges. The system is difficult to control because it is nonlinear, underactuated, involves hybrid dynamics due to slack-taut cable modes, and evolves on complex configuration spaces. Additionally, it is crucial to estimate the full state and the cable's mode transitions in real-time using on-board sensors and computation. To address these challenges, we present a novel Hybrid Perception-Aware Nonlinear Model Predictive Control (HPA-MPC) control approach for quadrotors with suspended loads. Our method considers the complete hybrid system dynamics and includes a perception-aware cost to ensure the payload remains visible in the robot's camera during navigation. Furthermore, the full state and hybrid dynamics' transitions are estimated using onboard sensors. Experimental results demonstrate that our approach enables stable load tracking control, even during slack-taut transitions, and operates entirely onboard. The experiments also show that the perception-aware term effectively keeps the payload in the robot's camera field of view when a human operator interacts with the load.

==> sections/archived.tex <==
highlight the necessity of a hybrid controller, 


% \begin{figure}[htbp]
%     \centering
%     \begin{minipage}[b]{0.13\columnwidth}
%         \centering
%         \includegraphics[width=\textwidth, trim=800 0 800 0, clip]{figures/nonhybrid_hover_gripper_gif/0.PNG} % Path to your image
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.13\columnwidth}
%         \centering
%         \includegraphics[width=\textwidth, trim=800 0 800 0, clip]{figures/nonhybrid_hover_gripper_gif/1.PNG} % image
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.13\columnwidth}
%         \centering
%         \includegraphics[width=\textwidth, trim=800 0 800 0, clip]{figures/nonhybrid_hover_gripper_gif/2.PNG} % image
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.13\columnwidth}
%         \centering
%         \includegraphics[width=\textwidth, trim=800 0 800 0, clip]{figures/nonhybrid_hover_gripper_gif/3.PNG} % image
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.13\columnwidth}
%         \centering
%         \includegraphics[width=\textwidth, trim=800 0 800 0, clip]{figures/nonhybrid_hover_gripper_gif/4.PNG} % image
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.13\columnwidth}
%         \centering
%         \includegraphics[width=\textwidth, trim=800 0 800 0, clip]{figures/nonhybrid_hover_gripper_gif/5.PNG} % image
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.13\columnwidth}
%         \centering
%         \includegraphics[width=\textwidth, trim=800 0 800 0, clip]{figures/nonhybrid_hover_gripper_gif/6.PNG} % image
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figures/plots_larger_font_v2/july_1_3_nohybrid_hover_manual_vertical_move.pdf}
%     \end{minipage}
%     \hfill
%     \caption{Non-Hybrid controller during a slack-taut transition in a hover scenario. The controller incorrectly commands the robot to move towards the payload during the slack state due to $z$ error in the desired payload position. We release the payload at $t=1.2$ to prevent a crash.}
%     \label{fig:non_hybrid_hover_gif}
% \end{figure}
% 
% \begin{figure}[htbp]
%     \centering
%     \begin{minipage}[b]{0.13\columnwidth}
%         \centering
%         \includegraphics[width=\textwidth, trim=200 0 200 0, clip]{figures/hybrid_hover_manual_gripper_gif/0.PNG} % Path to your image
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.13\columnwidth}
%         \centering
%         \includegraphics[width=\textwidth, trim=200 0 200 0, clip]{figures/hybrid_hover_manual_gripper_gif/1.PNG} % image
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.13\columnwidth}
%         \centering
%         \includegraphics[width=\textwidth, trim=200 0 200 0, clip]{figures/hybrid_hover_manual_gripper_gif/2.PNG} % image
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.13\columnwidth}
%         \centering
%         \includegraphics[width=\textwidth, trim=200 0 200 0, clip]{figures/hybrid_hover_manual_gripper_gif/3.PNG} % image
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.13\columnwidth}
%         \centering
%         \includegraphics[width=\textwidth, trim=200 0 200 0, clip]{figures/hybrid_hover_manual_gripper_gif/4.PNG} % image
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.13\columnwidth}
%         \centering
%         \includegraphics[width=\textwidth, trim=200 0 200 0, clip]{figures/hybrid_hover_manual_gripper_gif/5.PNG} % image
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.13\columnwidth}
%         \centering
%         \includegraphics[width=\textwidth, trim=200 0 200 0, clip]{figures/hybrid_hover_manual_gripper_gif/6.PNG} % image
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figures/plots_larger_font_v2/july_1_4_hybrid_hover_manual_vertical_move.pdf}
%     \end{minipage}
%     \caption{Hybrid controller during a slack-taut transition in a hover scenario. The robot maintains its position and is unaffected by the payload movement.}
%     \label{fig:hybrid_hover_gif}
% \end{figure}

\begin{figure*}
    \begin{minipage}[b]{1.5\columnwidth}
    \hspace{-10pt}
    \includegraphics[width=\textwidth, trim=100 250 100 300, clip]{figures/system_overview.pd}
    \end{minipage}
    \begin{minipage}[b]{0.55\columnwidth}
        \centering
        \includegraphics[width=\textwidth, trim=400 250 400 200, clip]{figures/system_convention_frames_2.pdf} \label{fig:figure1}
    \end{minipage}    
    \caption{(Left) The system architecture describing the flow of information through the various components of our pipeline. (Right) System Frame Convention}
    \label{fig:sys_overview}
\end{figure*}

==> sections/geom_control_and_traj_gen.tex <==
\section{Geometric Control and Trajectory Generation} 
\subsection{Nominal Geometric Controller}
We provide a brief overview of the well known geometric controller for a quadrotor attached to a point-mass suspended payload developed by \cite{sreenath2013cdc} and a simple payload trajectory generation scheme. Given a desired payload trajectory, the desired force acting on the payload is
\begin{align}
\vecF_{des} = &~\prths{m+\loadmass}\prths{\matK_{p}\vece_{\loadpos}+\matK_{d}\vece_{\loadvel}+\matK_{i}\int_0^t\vece_{\loadpos}d\tau}\nonumber\\
&~+\prths{m+\loadmass}\prths{\loadaccdes + \vecg}+ml\prths{\cabledotvec{}\cdot\cabledotvec{}}\cablevec{}, \label{eq:control-single-cable-plpos-control}
\end{align}
where $\matK_{p},\matK_{d},\matK_{i}\in\realnum{3\times3}$ are diagonal gain matrices and $\vece_{\loadpos},\vece_{\loadvel}\in\realnum{3}$ are the payload position and velocity errors defined as
\begin{equation}
\begin{split}
\vece_{\loadpos} = \loadposdes - \loadpos,\\
\vece_{\loadvel} = \loadveldes - \loadvel,~\label{eq:payload-pos-error}
\end{split}
\end{equation}
Since the desired force $\vecF_{des}$ is exerted by the tension cable, it defines the desired tension force vector. Hence the desired tension direction $\cablevec{des}$ can be obtained as
\begin{equation}
 \cablevec{des} = \frac{\vecF_{des}}{\twonorm{\vecF_{des}}}. 
\end{equation}
The thrust $f$ and moment $\matM$ acting on the quadrotor are
\begin{align}
f =& \vecF\cdot\robotrot{}\axis{3}{}\\
\vecF =&\cablevec{}\cablevec{}^\top\vecF_{des}-ml\cablevec{}\times\prths{\matK_{\cablevec{}}\vece_{\cablevec{}}+\matK_{\cablevel{}}\vece_{\cablevel{}}+\prths{\cablevec{}\cdot\cablevel{des}}\cabledotvec{}}\nonumber\\
~&+ml\cablevec{}\times\prths{\cablevec{des}\times\cableddotvec{des}},\label{eq:control-single-cable-qdthrust-control}
\end{align}
\begin{equation}
\begin{split}
\mathbf{M} =&~\matK_{R}\vece_{R} + \matK_{\Omega}\vece_{\Omega} + \robotangvel{}\times\inertia\robotangvel{}\\
&-\inertia\prths{\hat{\robotangvel{}}\robotrot{}^{\top}\robotrot{des}\robotangvel{des}-\robotrot{}^{\top}\robotrot{des}\dot{\robotangvel{}}_{des}},\label{eq:control-single-cable-qdatt-control}
\end{split}
\end{equation}
where $\matK_{R},\matK_{\Omega},\matK_{\cablevec{}},\matK_{\cablevel{}}\in\realnum{3\times3}$ are diagonal gain matrices, $\vece_{R} , \vece_{\Omega}\in\realnum{3}$ are quadrotor's orientation, angular velocity errors defined as
\begin{equation}
\begin{split}
\vece_{\robotrot{}} &= \half\prths{\robotrot{}^{\top}\robotrot{des}-\robotrot{des}^{\top}\robotrot{}}^{\vee}, \\
\vece_{\robotangvel{}} &=  \robotrot{}^{\top}\robotrot{des}\robotangvel{des} - \robotangvel{},\label{eq:robot-angular-error}
\end{split}
\end{equation}
and $ \vece_{\cablevec{}}, \vece_{\cablevel{}}\in\realnum{3}$ are cable direction, cable velocity errors defined as
\begin{equation}
\vece_{\cablevec{}}= \cablevec{des} \times\cablevec{},~
\vece_{\cablevel{}} = \cablevel{} + \cablevec{}\times
\cablevec{}\times\cablevel{des}.\label{eq:cable-error}
\end{equation}

\subsection{Trajectory Generation}
We validate our NMPC method to track lissajous payload trajectories that are generated using the following equations
\begin{equation}
\loadposdes(t) = \begin{bmatrix}
    a\sin(t)&b\sin(nt + \phi)&c\sin(mt) + \psi    \label{eq:lissajous_traj_eq}
\end{bmatrix}^\top
\end{equation}
where $n,m$ control the relative periods of $x,y,z$ motions and $a,b$ and $c$ their relative amplitudes. By differentiating \eqref{eq:lissajous_traj_eq}, we obtain $\loadveldes(t)$ and $\loadaccdes(t)$. \\

As we will see in section x.x, it will be useful to know the nominal $\robotdes(t)$ and $\matR_{des} (t)$, which can be calculated using the system's differential flatness properties as shown in \cite{sreenath2013geometric}.

# talk about angular rates
